Learning Model Predictive Control for Quadrotors

Aerial robots can enhance their safe and agile navigation in complex and cluttered environments by efficiently exploiting the information collected during a given task. In this paper, we address the learning model predictive control problem for quadrotors. We design a learning receding--horizon nonlinear control strategy directly formulated on the system nonlinear manifold configuration space SO(3)xR^3. The proposed approach exploits past successful task iterations to improve the system performance over time while respecting system dynamics and actuator constraints. We further relax its computational complexity making it compatible with real-time quadrotor control requirements. We show the effectiveness of the proposed approach in learning a minimum time control task, respecting dynamics, actuators, and environment constraints. Several experiments in simulation and real-world set-up validate the proposed approach.

==> symbol_list.tex <==
%!TEX root = ARTICLE.tex
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathOperator{\Diag}{Diag} 
%%%%%%%%%%%%% Comando para glosario %%%%%%%%%%%%%%55
\newcommand{\glo}[3]{
%#1: id
%#2: name
%#3: 
	\newglossaryentry{#1}
	{
	  name=#2,
	  description=#3,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glom}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  type=symbols,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glomh}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  %type=hidden,
	}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\glo{naiive}{naive}{ratio of circumference of circle to its
               diameter}



%%http://tex.stackexchange.com/questions/236670/custom-glossary-style-makenoidxglossaries-and-glsgroupskip


%% Linear model
\glomh{linx}{A}{A}{Input matrix.}
\glomh{linp}{C}{C}{parameter matrix.}


% dynamics
\glom{sgn}{\chi}{\chi}{Indicator function}
\glom{error}{e}{e}{Desired roll}
% \glom{droll}{\phi^*}{\phi^*}{Desired roll}
\glom{roll}{\phi}{\phi}{roll}
\glom{pitch}{\theta}{\theta}{pitch}
\glom{yaw}{\psi}{\psi}{yaw}
\glom{droll}{ p}{ p}{roll}
\glom{dpitch}{ q}{ q}{pitch}
\glom{dyaw}{ r}{ r}{yaw}
\glom{angles}{\mathbf{\Theta}}{\mathbf{\Theta}}{Robot attitude}
\glom{dangles}{\mathbf{\Omega}}{\mathbf{\Omega}}{Angular velocities}
\glom{id}{k}{k}{general id of robot used in description of control method and estimation}

\glom{thrust}{F}{F}{Thrust}
\glom{u}{\mathbf{u}}{\mathbf{u}}{control input}
\glom{w}{\mathbf{w}}{\mathbf{w}}{control input}
\glom{angular}{\omega}{\omega}{angular speed}

% Coordinate frames
\glom{worldf}{\mathcal{I}}{\mathcal{I}}{World frame}
\glom{loadf}{\mathcal{L}}{\mathcal{L}}{Load frame}
\glom{robotf}{\mathcal{B}}{\mathcal{B}}{Body frame}
\glom{camf}{\mathcal{C}}{\mathcal{C}}{Camera frame}

%\glom{tagf}{\mathpzc{T}}{\mathpzc{T}}{Tag frame}
%\glom{dockf}{\mathpzc{d}}{\mathpzc{d}}{Docking module frame}
%\glom{camf}{\mathpzc{C}}{\mathpzc{C}}{Camera frame}
%\glom{waitf}{\mathpzc{w}}{\mathpzc{w}}{Waiting module frame}

%% Robots
\glom{tag}{\mathpzc{t}_p}{\mathpzc{t}_p}{Tag}
\glom{robots}{\mathcal{R}}{\mathcal{R}}{Set of a team of robots}
\glom{robotl}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{robot}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{width}{\mathpzc{w}}{\mathpzc{w}}{Robot width.}
\glom{height}{\mathpzc{h}}{\mathpzc{h}}{Robot height.}
\glom{orientations}{\Psi}{\Psi}{Robot orientations.}
\glom{orientation}{\psi}{\psi}{Robot orientation.}
\glom{structure}{\mathit{S}}{\mathit{S}}{Structure}
\glom{structureset}{\mathcal{S_F}}{\mathcal{S_F}}{Structure set}
\glom{component}{\mathit{S}}{\mathit{S}}{Structure}

% Desired structure
\glom{targets}{\mathcal{Z}}{\mathcal{Z}}{Target points}
\glom{targetse}{\mathcal{Z}^E}{\mathcal{Z}^E}{Expanded target points}
\glom{target}{z}{z}{Robot location.}

\glom{tree}{\mathcal{T}}{\mathcal{T}}{Assembly tree.}
\glom{tedges}{\mathcal{E}^\mathcal{T}}{\mathcal{E}^\mathcal{T}}{Edges of the Assembly tree.}
\glom{tvertices}{\mathcal{V}^\mathcal{T}}{\mathcal{V}^\mathcal{T}}{Vertices of the Assembly tree.}
\glom{tivertices}{\mathcal{V}^{\mathcal{T}_i}}{\mathcal{V}^{\mathcal{T}_i}}{Vertices of the Assembly tree.}

\glom{graph}{\mathcal{G}}{\mathcal{G}}{Communication graph}
\glom{cgraph}{\hat{\mathcal{G}}}{\hat{\mathcal{G}}}{Canonical robust graph}
\glom{vertices}{\mathcal{V}}{\mathcal{V}}{Set of Vertices}
\glom{neighbors}{\mathcal{N}_i}{\mathcal{N}}{Neighbors for node $i$}
\glom{edges}{\mathcal{E}}{\mathcal{E}}{Set of Edges}
\glom{neighborsi}{\mathcal{J}_i}{\mathcal{J}}{Inclusive Neighbors for node $i$}
\glom{removed}{\mathcal{R}}{\mathcal{R}}{Removed nodes}
\glom{normal}{\mathcal{N}}{\mathcal{N}}{Normal nodes}
\glom{strongset}{\mathcal{F}}{\mathcal{F}}{Strong nodes}
\glom{weakset}{\mathcal{W}}{\mathcal{W}}{Weak nodes}
\glom{candidates}{\mathcal{C}}{\mathcal{C}}{Candidate points}
\glom{boundary}{\mathcal{P}}{\mathcal{P}}{Objective points}

\glom{loc}{v}{v}{Node location in the space}
\glom{val}{x}{x}{Variable of interest of the node}

\glom{received}{\mathcal{P}_i^t}{\mathcal{P}}{Set of received values by node $i$ a the time interval 
%$[t-T\, t]$
}


